O(1) Communication for Distributed SGD through Two-Level Gradient Averaging

Large neural network models present a hefty communication challenge to distributed Stochastic Gradient Descent (SGD), with a communication complexity of O(n) per worker for a model of n parameters. Many sparsification and quantization techniques have been proposed to compress the gradients, some reducing the communication complexity to O(k), where k << n. In this paper, we introduce a strategy called two-level gradient averaging (A2SGD) to consolidate all gradients down to merely two local averages per worker before the computation of two global averages for an updated model. A2SGD also retains local errors to maintain the variance for fast convergence. Our theoretical analysis shows that A2SGD converges similarly like the default distributed SGD algorithm. Our evaluation validates the theoretical conclusion and demonstrates that A2SGD significantly reduces the communication traffic per worker, and improves the overall training time of LSTM-PTB by 3.2x and 23.2x, respectively, compared to Top-K and QSGD. To the best of our knowledge, A2SGD is the first to achieve O(1) communication complexity per worker for distributed SGD.

==> evaluation/acc_loss/script_acc <==
python ../plot.py --network FNN3 --plot-type accuracy --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/fcn5net-n8-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/fcn5net-n8-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/fcn5net-n8-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/fcn5net-n8-*/*-0.log --legends Dense TopK QSGD A2SGD

python ../plot.py --network ResNet20 --plot-type accuracy --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/resnet20-n8-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/resnet20-n8-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/resnet20-n8-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/resnet20-n8-*/*-0.log --legends Dense TopK QSGD A2SGD

python ../plot.py --network LSTM --plot-type accuracy --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/lstm-n8-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/lstm-n8-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/lstm-n8-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/lstm-n8-*/*-0.log --legends Dense TopK QSGD A2SGD

python ../plot.py --network VGG16 --plot-type accuracy --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/vgg16-n8-*/*-0.log  \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/vgg16-n8-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/vgg16-n8-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/vgg16-n8-*/*-0.log --legends Dense TopK QSGD A2SGD



==> evaluation/acc_loss/script_acc_gaussian <==

python ../plot.py --network FNN3-16 --plot-type accuracy --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/fcn5net-n16-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/fcn5net-n16-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/fcn5net-n16-*/*-0.log ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/fcn5net-n16-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/fcn5net-n16-*/*-0.log --legends Dense TopK QSGD GaussianK A2SGD

python ../plot.py --network FNN3-8 --plot-type accuracy --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/fcn5net-n8-*/*-0.log \
 ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/fcn5net-n8-*/*-0.log ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/fcn5net-n8-*/*-0.log ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/fcn5net-n8-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/fcn5net-n8-*/*-0.log --legends Dense TopK QSGD GaussianK A2SGD

python ../plot.py --network FNN3-4 --plot-type accuracy --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/fcn5net-n4-*/*-0.log \
 ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/fcn5net-n4-*/*-0.log ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/fcn5net-n4-*/*-0.log ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/fcn5net-n4-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/fcn5net-n4-*/*-0.log --legends Dense TopK QSGD GaussianK A2SGD

python ../plot.py --network FNN3-2 --plot-type accuracy --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/fcn5net-n2-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/fcn5net-n2-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/fcn5net-n2-*/*-0.log ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/fcn5net-n2-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/fcn5net-n2-*/*-0.log --legends Dense TopK QSGD GaussianK A2SGD

python ../plot.py --network ResNet20-16 --plot-type accuracy --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/resnet20-n16-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/resnet20-n16-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/resnet20-n16-*/*-0.log ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/resnet20-n16-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/resnet20-n16-*/*-0.log --legends Dense TopK QSGD GaussianK A2SGD

python ../plot.py --network ResNet20-8 --plot-type accuracy --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/resnet20-n8-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/resnet20-n8-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/resnet20-n8-*/*-0.log ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/resnet20-n8-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/resnet20-n8-*/*-0.log --legends Dense TopK QSGD GaussianK A2SGD

python ../plot.py --network ResNet20-4 --plot-type accuracy --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/resnet20-n4-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/resnet20-n4-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/resnet20-n4-*/*-0.log ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/resnet20-n4-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/resnet20-n4-*/*-0.log --legends Dense TopK QSGD GaussianK A2SGD

python ../plot.py --network ResNet20-2 --plot-type accuracy --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/resnet20-n2-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/resnet20-n2-*/*-0.log ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/resnet20-n2-*/*-0.log \
 ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/resnet20-n2-*/*-0.log ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/resnet20-n2-*/*-0.log --legends Dense TopK QSGD GaussianK A2SGD

python ../plot.py --network LSTM-16 --plot-type accuracy --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/lstm-n16-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/lstm-n16-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/lstm-n16-*/*-0.log ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/lstm-n16-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/lstm-n16-*/*-0.log --legends Dense TopK QSGD GaussianK A2SGD

python ../plot.py --network LSTM-8 --plot-type accuracy --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/lstm-n8-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/lstm-n8-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/lstm-n8-*/*-0.log ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/lstm-n8-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/lstm-n8-*/*-0.log --legends Dense TopK QSGD GaussianK A2SGD

python ../plot.py --network LSTM-4 --plot-type accuracy --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/lstm-n4-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/lstm-n4-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/lstm-n4-*/*-0.log ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/lstm-n4-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/lstm-n4-*/*-0.log --legends Dense TopK QSGD GaussianK A2SGD

python ../plot.py --network LSTM-2 --plot-type accuracy --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/lstm-n2-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/lstm-n2-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/lstm-n2-*/*-0.log ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/lstm-n2-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/lstm-n2-*/*-0.log --legends Dense TopK QSGD GaussianK A2SGD

python ../plot.py --network VGG16-16 --plot-type accuracy --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/vgg16-n16-*/*-0.log  \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/vgg16-n16-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/vgg16-n16-*/*-0.log ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/vgg16-n16-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/vgg16-n16-*/*-0.log --legends Dense TopK QSGD GaussianK A2SGD

python ../plot.py --network VGG16-8 --plot-type accuracy --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/vgg16-n8-*/*-0.log  \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/vgg16-n8-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/vgg16-n8-*/*-0.log ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/vgg16-n8-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/vgg16-n8-*/*-0.log --legends Dense TopK QSGD GaussianK A2SGD

python ../plot.py --network VGG16-4 --plot-type accuracy --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/vgg16-n4-*/*-0.log  \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/vgg16-n4-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/vgg16-n4-*/*-0.log ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/vgg16-n4-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/vgg16-n4-*/*-0.log --legends Dense TopK QSGD GaussianK A2SGD

python ../plot.py --network VGG16-2 --plot-type accuracy --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/vgg16-n2-*/*-0.log  \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/vgg16-n2-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/vgg16-n2-*/*-0.log ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/vgg16-n2-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/vgg16-n2-*/*-0.log --legends Dense TopK QSGD GaussianK A2SGD



==> evaluation/acc_loss/script_loss <==
python ../plot.py --network FNN3 --plot-type loss --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/fcn5net-n8-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/fcn5net-n8-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/fcn5net-n8-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/fcn5net-n8-*/*-0.log --legends Dense TopK QSGD A2SGD

python ../plot.py --network ResNet20 --plot-type loss --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/resnet20-n8-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/resnet20-n8-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/resnet20-n8-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/resnet20-n8-*/*-0.log --legends Dense TopK QSGD A2SGD

python ../plot.py --network LSTM --plot-type loss --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/lstm-n8-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/lstm-n8-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/lstm-n8-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/lstm-n8-*/*-0.log --legends Dense TopK QSGD A2SGD

python ../plot.py --network VGG16 --plot-type loss --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/vgg16-n8-*/*-0.log  \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/vgg16-n8-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/vgg16-n8-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/vgg16-n8-*/*-0.log --legends Dense TopK QSGD A2SGD



==> evaluation/acc_loss/script_loss_gaussian <==

python ../plot.py --network FNN3-16 --plot-type loss --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/fcn5net-n16-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/fcn5net-n16-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/fcn5net-n16-*/*-0.log ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/fcn5net-n16-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/fcn5net-n16-*/*-0.log --legends Dense TopK QSGD GaussianK A2SGD

python ../plot.py --network FNN3-8 --plot-type loss --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/fcn5net-n8-*/*-0.log \
 ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/fcn5net-n8-*/*-0.log ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/fcn5net-n8-*/*-0.log ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/fcn5net-n8-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/fcn5net-n8-*/*-0.log --legends Dense TopK QSGD GaussianK A2SGD

python ../plot.py --network FNN3-4 --plot-type loss --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/fcn5net-n4-*/*-0.log \
 ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/fcn5net-n4-*/*-0.log ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/fcn5net-n4-*/*-0.log ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/fcn5net-n4-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/fcn5net-n4-*/*-0.log --legends Dense TopK QSGD GaussianK A2SGD

python ../plot.py --network FNN3-2 --plot-type loss --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/fcn5net-n2-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/fcn5net-n2-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/fcn5net-n2-*/*-0.log ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/fcn5net-n2-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/fcn5net-n2-*/*-0.log --legends Dense TopK QSGD GaussianK A2SGD

python ../plot.py --network ResNet20-16 --plot-type loss --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/resnet20-n16-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/resnet20-n16-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/resnet20-n16-*/*-0.log ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/resnet20-n16-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/resnet20-n16-*/*-0.log --legends Dense TopK QSGD GaussianK A2SGD

python ../plot.py --network ResNet20-8 --plot-type loss --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/resnet20-n8-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/resnet20-n8-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/resnet20-n8-*/*-0.log ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/resnet20-n8-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/resnet20-n8-*/*-0.log --legends Dense TopK QSGD GaussianK A2SGD

python ../plot.py --network ResNet20-4 --plot-type loss --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/resnet20-n4-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/resnet20-n4-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/resnet20-n4-*/*-0.log ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/resnet20-n4-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/resnet20-n4-*/*-0.log --legends Dense TopK QSGD GaussianK A2SGD

python ../plot.py --network ResNet20-2 --plot-type loss --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/resnet20-n2-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/resnet20-n2-*/*-0.log ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/resnet20-n2-*/*-0.log \
 ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/resnet20-n2-*/*-0.log ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/resnet20-n2-*/*-0.log --legends Dense TopK QSGD GaussianK A2SGD

python ../plot.py --network LSTM-16 --plot-type loss --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/lstm-n16-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/lstm-n16-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/lstm-n16-*/*-0.log ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/lstm-n16-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/lstm-n16-*/*-0.log --legends Dense TopK QSGD GaussianK A2SGD

python ../plot.py --network LSTM-8 --plot-type loss --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/lstm-n8-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/lstm-n8-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/lstm-n8-*/*-0.log ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/lstm-n8-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/lstm-n8-*/*-0.log --legends Dense TopK QSGD GaussianK A2SGD

python ../plot.py --network LSTM-4 --plot-type loss --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/lstm-n4-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/lstm-n4-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/lstm-n4-*/*-0.log ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/lstm-n4-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/lstm-n4-*/*-0.log --legends Dense TopK QSGD GaussianK A2SGD

python ../plot.py --network LSTM-2 --plot-type loss --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/lstm-n2-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/lstm-n2-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/lstm-n2-*/*-0.log ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/lstm-n2-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/lstm-n2-*/*-0.log --legends Dense TopK QSGD GaussianK A2SGD

python ../plot.py --network VGG16-16 --plot-type loss --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/vgg16-n16-*/*-0.log  \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/vgg16-n16-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/vgg16-n16-*/*-0.log ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/vgg16-n16-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/vgg16-n16-*/*-0.log --legends Dense TopK QSGD GaussianK A2SGD

python ../plot.py --network VGG16-8 --plot-type loss --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/vgg16-n8-*/*-0.log  \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/vgg16-n8-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/vgg16-n8-*/*-0.log ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/vgg16-n8-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/vgg16-n8-*/*-0.log --legends Dense TopK QSGD GaussianK A2SGD

python ../plot.py --network VGG16-4 --plot-type loss --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/vgg16-n4-*/*-0.log  \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/vgg16-n4-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/vgg16-n4-*/*-0.log ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/vgg16-n4-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/vgg16-n4-*/*-0.log --legends Dense TopK QSGD GaussianK A2SGD

python ../plot.py --network VGG16-2 --plot-type loss --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/vgg16-n2-*/*-0.log  \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/vgg16-n2-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/vgg16-n2-*/*-0.log ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/vgg16-n2-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/vgg16-n2-*/*-0.log --legends Dense TopK QSGD GaussianK A2SGD



==> evaluation/convergence/convergence_fnn3 <==
python ../plot.py --network FNN3-16worker --plot-type loss --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/fcn5net-n16-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/fcn5net-n16-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/fcn5net-n16-*/*-0.log \
../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/fcn5net-n16-*/*-0.log --legends Dense TopK QSGD A2SGD

python ../plot.py --network FNN3-8worker --plot-type loss --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/fcn5net-n8-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/fcn5net-n8-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/fcn5net-n8-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/fcn5net-n8-*/*-0.log --legends Dense TopK QSGD A2SGD

python ../plot.py --network FNN3-4worker --plot-type loss --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/fcn5net-n4-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/fcn5net-n4-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/fcn5net-n16-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/fcn5net-n4-*/*-0.log --legends Dense TopK QSGD A2SGD

python ../plot.py --network FNN3-2worker --plot-type loss --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/fcn5net-n2-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/fcn5net-n2-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/fcn5net-n16-*/*-0.log \
 \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/fcn5net-n2-*/*-0.log --legends Dense TopK QSGD A2SGD

python ../plot.py --network FNN3-16worker --plot-type accuracy --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/fcn5net-n16-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/fcn5net-n16-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/fcn5net-n16-*/*-0.log \
../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/fcn5net-n16-*/*-0.log --legends Dense TopK QSGD A2SGD

python ../plot.py --network FNN3-8worker --plot-type accuracy --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/fcn5net-n8-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/fcn5net-n8-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/fcn5net-n8-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/fcn5net-n8-*/*-0.log --legends Dense TopK QSGD A2SGD

python ../plot.py --network FNN3-4worker --plot-type accuracy --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/fcn5net-n4-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/fcn5net-n4-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/fcn5net-n16-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/fcn5net-n4-*/*-0.log --legends Dense TopK QSGD A2SGD

python ../plot.py --network FNN3-2worker --plot-type accuracy --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/fcn5net-n2-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/fcn5net-n2-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/fcn5net-n16-*/*-0.log \
 \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/fcn5net-n2-*/*-0.log --legends Dense TopK QSGD A2SGD 

==> evaluation/convergence/convergence_lstm <==
python ../plot.py --network LSTM-16worker --plot-type loss --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/lstm-n16-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/lstm-n16-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/lstm-n16-*/*-0.log \
../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/lstm-n16-*/*-0.log --legends Dense TopK QSGD A2SGD

python ../plot.py --network LSTM-8worker --plot-type loss --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/lstm-n8-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/lstm-n8-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/lstm-n8-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/lstm-n8-*/*-0.log --legends Dense TopK QSGD A2SGD

python ../plot.py --network LSTM-4worker --plot-type loss --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/lstm-n4-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/lstm-n4-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/lstm-n16-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/lstm-n4-*/*-0.log --legends Dense TopK QSGD A2SGD

python ../plot.py --network LSTM-2worker --plot-type loss --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/lstm-n2-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/lstm-n2-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/lstm-n16-*/*-0.log \
 \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/lstm-n2-*/*-0.log --legends Dense TopK QSGD A2SGD

python ../plot.py --network LSTM-16worker --plot-type accuracy --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/lstm-n16-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/lstm-n16-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/lstm-n16-*/*-0.log \
../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/lstm-n16-*/*-0.log --legends Dense TopK QSGD A2SGD

python ../plot.py --network LSTM-8worker --plot-type accuracy --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/lstm-n8-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/lstm-n8-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/lstm-n8-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/lstm-n8-*/*-0.log --legends Dense TopK QSGD A2SGD

python ../plot.py --network LSTM-4worker --plot-type accuracy --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/lstm-n4-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/lstm-n4-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/lstm-n16-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/lstm-n4-*/*-0.log --legends Dense TopK QSGD A2SGD

python ../plot.py --network LSTM-2worker --plot-type accuracy --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/lstm-n2-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/lstm-n2-*/*-0.log  ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/lstm-n16-*/*-0.log \
 \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/lstm-n2-*/*-0.log --legends Dense TopK QSGD A2SGD

==> evaluation/convergence/convergence_resnet20 <==
python ../plot.py --network ResNet20-16worker --plot-type loss --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/resnet20-n16-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/resnet20-n16-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/resnet20-n16-*/*-0.log \
../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/resnet20-n16-*/*-0.log --legends Dense TopK QSGD A2SGD

python ../plot.py --network ResNet20-8worker --plot-type loss --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/resnet20-n8-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/resnet20-n8-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/resnet20-n8-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/resnet20-n8-*/*-0.log --legends Dense TopK QSGD A2SGD

python ../plot.py --network ResNet20-4worker --plot-type loss --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/resnet20-n4-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/resnet20-n4-*/*-0.log  ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/resnet20-n16-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/resnet20-n4-*/*-0.log --legends Dense TopK QSGD A2SGD

python ../plot.py --network ResNet20-2worker --plot-type loss --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/resnet20-n2-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/resnet20-n2-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/resnet20-n16-*/*-0.log \
 \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/resnet20-n2-*/*-0.log --legends Dense TopK QSGD A2SGD

python ../plot.py --network ResNet20-16worker --plot-type accuracy --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/resnet20-n16-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/resnet20-n16-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/resnet20-n16-*/*-0.log \
../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/resnet20-n16-*/*-0.log --legends Dense TopK QSGD A2SGD

python ../plot.py --network ResNet20-8worker --plot-type accuracy --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/resnet20-n8-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/resnet20-n8-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/resnet20-n8-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/resnet20-n8-*/*-0.log --legends Dense TopK QSGD A2SGD

python ../plot.py --network ResNet20-4worker --plot-type accuracy --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/resnet20-n4-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/resnet20-n4-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/resnet20-n16-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/resnet20-n4-*/*-0.log --legends Dense TopK QSGD A2SGD

python ../plot.py --network ResNet20-2worker --plot-type accuracy --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/resnet20-n2-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/resnet20-n2-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/resnet20-n16-*/*-0.log \
 \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/resnet20-n2-*/*-0.log --legends Dense TopK QSGD A2SGD

==> evaluation/convergence/convergence_vgg16 <==
python ../plot.py --network VGG16-16worker --plot-type loss --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/vgg16-n16-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/vgg16-n16-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/vgg16-n16-*/*-0.log \
../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/vgg16-n16-*/*-0.log --legends Dense TopK QSGD A2SGD

python ../plot.py --network VGG16-8worker --plot-type loss --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/vgg16-n8-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/vgg16-n8-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/vgg16-n8-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/vgg16-n8-*/*-0.log --legends Dense TopK QSGD A2SGD

python ../plot.py --network VGG16-4worker --plot-type loss --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/vgg16-n4-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/vgg16-n4-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/vgg16-n16-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/vgg16-n4-*/*-0.log --legends Dense TopK QSGD A2SGD

python ../plot.py --network VGG16-2worker --plot-type loss --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/vgg16-n2-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/vgg16-n2-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/vgg16-n16-*/*-0.log \
 \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/vgg16-n2-*/*-0.log --legends Dense TopK QSGD A2SGD

python ../plot.py --network VGG16-16worker --plot-type accuracy --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/vgg16-n16-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/vgg16-n16-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/vgg16-n16-*/*-0.log \
../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/vgg16-n16-*/*-0.log --legends Dense TopK QSGD A2SGD

python ../plot.py --network VGG16-8worker --plot-type accuracy --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/vgg16-n8-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/vgg16-n8-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/vgg16-n8-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/vgg16-n8-*/*-0.log --legends Dense TopK QSGD A2SGD

python ../plot.py --network VGG16-4worker --plot-type accuracy --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/vgg16-n4-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/vgg16-n4-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/vgg16-n16-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/vgg16-n4-*/*-0.log --legends Dense TopK QSGD A2SGD

python ../plot.py --network VGG16-2worker --plot-type accuracy --logfile-name ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/vgg16-n2-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/vgg16-n2-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/vgg16-n16-*/*-0.log \
 \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/vgg16-n2-*/*-0.log --legends Dense TopK QSGD A2SGD

==> evaluation/speedup/script_speedup <==
#Need to fix topk(2, 4) and None(2)
python ../plot_speedup.py ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/resnet20-n2-*/*-0.log ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/resnet20-n4-*/*-0.log \
 ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/resnet20-n8-*/*-0.log ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/resnet20-n16-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/resnet20-n2-*/*-0.log ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/resnet20-n4-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/resnet20-n8-*/*-0.log ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/resnet20-n16-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/resnet20-n2-*/*-0.log ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/resnet20-n4-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/resnet20-n8-*/*-0.log ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/resnet20-n16-*/*-0.log \
 ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/resnet20-n2-*/*-0.log ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/resnet20-n4-*/*-0.log \
 ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/resnet20-n8-*/*-0.log ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/resnet20-n16-*/*-0.log \
 ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/resnet20-n2-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/resnet20-n4-*/*-0.log \
 ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/resnet20-n8-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/resnet20-n16-*/*-0.log ResNet20_speedup

 python ../plot_speedup.py ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/vgg16-n2-*/*-0.log ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/vgg16-n4-*/*-0.log \
 ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/vgg16-n8-*/*-0.log ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/vgg16-n16-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/vgg16-n2-*/*-0.log ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/vgg16-n4-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/vgg16-n8-*/*-0.log ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/vgg16-n16-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/vgg16-n2-*/*-0.log ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/vgg16-n4-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/vgg16-n8-*/*-0.log ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/vgg16-n16-*/*-0.log \
 ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/vgg16-n2-*/*-0.log ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/vgg16-n4-*/*-0.log \
 ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/vgg16-n8-*/*-0.log ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/vgg16-n16-*/*-0.log \
 ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/vgg16-n2-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/vgg16-n4-*/*-0.log \
 ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/vgg16-n8-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/vgg16-n16-*/*-0.log VGG16_speedup

 python ../plot_speedup.py ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/lstm-n2-*/*-0.log ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/lstm-n4-*/*-0.log \
 ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/lstm-n8-*/*-0.log ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/lstm-n16-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/lstm-n2-*/*-0.log ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/lstm-n4-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/lstm-n8-*/*-0.log ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/lstm-n16-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/lstm-n2-*/*-0.log ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/lstm-n4-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/lstm-n8-*/*-0.log ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/lstm-n16-*/*-0.log \
 ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/lstm-n2-*/*-0.log ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/lstm-n4-*/*-0.log \
 ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/lstm-n8-*/*-0.log ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/lstm-n16-*/*-0.log \
 ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/lstm-n2-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/lstm-n4-*/*-0.log \
 ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/lstm-n8-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/lstm-n16-*/*-0.log LSTM_speedup
  
 python ../plot_speedup.py ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/fcn5net-n2-*/*-0.log ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/fcn5net-n4-*/*-0.log \
 ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/fcn5net-n8-*/*-0.log ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/fcn5net-n16-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/fcn5net-n2-*/*-0.log ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/fcn5net-n4-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/fcn5net-n8-*/*-0.log ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/fcn5net-n16-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/fcn5net-n2-*/*-0.log ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/fcn5net-n4-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/fcn5net-n8-*/*-0.log ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/fcn5net-n16-*/*-0.log \
 ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/fcn5net-n2-*/*-0.log ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/fcn5net-n4-*/*-0.log \
 ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/fcn5net-n8-*/*-0.log ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/fcn5net-n16-*/*-0.log \
 ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/fcn5net-n2-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/fcn5net-n4-*/*-0.log \
 ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/fcn5net-n8-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/fcn5net-n16-*/*-0.log FNN3_speedup

==> evaluation/walltime/script_time <==
#Need to fix topk(2, 4) and None(2)
python ../plot_time.py ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/resnet20-n2-*/*-0.log ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/resnet20-n4-*/*-0.log \
 ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/resnet20-n8-*/*-0.log ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/resnet20-n16-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/resnet20-n2-*/*-0.log ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/resnet20-n4-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/resnet20-n8-*/*-0.log ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/resnet20-n16-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/resnet20-n2-*/*-0.log ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/resnet20-n4-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/resnet20-n8-*/*-0.log ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/resnet20-n16-*/*-0.log \
 ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/resnet20-n2-*/*-0.log ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/resnet20-n4-*/*-0.log \
 ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/resnet20-n8-*/*-0.log ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/resnet20-n16-*/*-0.log \
 ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/resnet20-n2-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/resnet20-n4-*/*-0.log \
 ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/resnet20-n8-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/resnet20-n16-*/*-0.log ResNet20_time

 python ../plot_time.py ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/vgg16-n2-*/*-0.log ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/vgg16-n4-*/*-0.log \
 ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/vgg16-n8-*/*-0.log ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/vgg16-n16-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/vgg16-n2-*/*-0.log ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/vgg16-n4-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/vgg16-n8-*/*-0.log ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/vgg16-n16-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/vgg16-n2-*/*-0.log ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/vgg16-n4-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/vgg16-n8-*/*-0.log ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/vgg16-n16-*/*-0.log \
 ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/vgg16-n2-*/*-0.log ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/vgg16-n4-*/*-0.log \
 ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/vgg16-n8-*/*-0.log ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/vgg16-n16-*/*-0.log \
 ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/vgg16-n2-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/vgg16-n4-*/*-0.log \
 ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/vgg16-n8-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/vgg16-n16-*/*-0.log VGG16_time

 python ../plot_time.py ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/lstm-n2-*/*-0.log ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/lstm-n4-*/*-0.log \
 ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/lstm-n8-*/*-0.log ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/lstm-n16-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/lstm-n2-*/*-0.log ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/lstm-n4-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/lstm-n8-*/*-0.log ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/lstm-n16-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/lstm-n2-*/*-0.log ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/lstm-n4-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/lstm-n8-*/*-0.log ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/lstm-n16-*/*-0.log \
 ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/lstm-n2-*/*-0.log ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/lstm-n4-*/*-0.log \
 ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/lstm-n8-*/*-0.log ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/lstm-n16-*/*-0.log \
 ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/lstm-n2-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/lstm-n4-*/*-0.log \
 ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/lstm-n8-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/lstm-n16-*/*-0.log LSTM_time
  
 python ../plot_time.py ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/fcn5net-n2-*/*-0.log ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/fcn5net-n4-*/*-0.log \
 ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/fcn5net-n8-*/*-0.log ../allreduce-comp-none-gwarmup-convergence-thres-512000kbytes/fcn5net-n16-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/fcn5net-n2-*/*-0.log ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/fcn5net-n4-*/*-0.log \
 ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/fcn5net-n8-*/*-0.log ../allreduce-comp-topk-gwarmup-convergence-thres-512000kbytes/fcn5net-n16-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/fcn5net-n2-*/*-0.log ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/fcn5net-n4-*/*-0.log \
 ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/fcn5net-n8-*/*-0.log ../allreduce-comp-fsgd-gwarmup-convergence-thres-512000kbytes/fcn5net-n16-*/*-0.log \
 ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/fcn5net-n2-*/*-0.log ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/fcn5net-n4-*/*-0.log \
 ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/fcn5net-n8-*/*-0.log ../allreduce-comp-gaussian-gwarmup-convergence-thres-512000kbytes/fcn5net-n16-*/*-0.log \
 ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/fcn5net-n2-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/fcn5net-n4-*/*-0.log \
 ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/fcn5net-n8-*/*-0.log ../allreduce-comp-qsgd-gwarmup-convergence-thres-512000kbytes/fcn5net-n16-*/*-0.log FNN3_time

==> text/convergence.tex <==
\subsection{Convergence Rate}

\begin{comment}
Detecting gradient bound --

First consider the mean and variance of the bell-shaped curve used in Vanilla 
distributed SGD with gradient vector $g_t^P$-

Mean of the gradient distribution: $\mu_1 = \frac{1}{P}\sum_{p=1}^{P}g_t^p$ = 
Gradient produced in Dense SGD

Variance of the gradient distribution: $\sigma_1 = \parallel g_t^P \parallel^2$


%Now calculate the mean and variance of our distribution:

%Using Eq:~\ref{eq:4}, we will calculate the mean and variance of our 
%distribution of gradient vector-

Now, we will calculate the exact distance between the spread of Dense SGD and 
\brand

$\mu_2 = g_t^P - \Aop(g_t^P) + \frac{1}{P}\sum_{P=1}^P \Aop (g^p_t)$

Variance of \brand gradient distribution: $\sigma_2 = \parallel g_t^P 
\parallel^2$ 
as variance of $\Aop$ operator is zero as it returns mean always.

distance between the two spread(Dense SGD in distributed node and $\Aop$) then 
can be calculated as-
distance$= (\mu_1 + 2\sigma_1) - (\mu_2 + 2\sigma_2)  = (\mu_1 - \mu_2)$

\begin{equation}
= g_t^P - (g_t^P - 
\Aop(g_t^P) + \frac{1}{P}\sum_{P=1}^P \Aop (g^p_t))
\end{equation}
\begin{equation}
=\{\frac{g_t^P}{\parallel g^P_t \parallel^2} - 1 +
\frac{\Aop(g_t^P)}{\parallel g^P_t \parallel^2} - 
\frac{\frac{1}{P}\sum_{p=1}^{P}\Aop(g_t^p)}{\parallel g^P_t \parallel^2}\} 
\parallel g^P_t \parallel^2
\end{equation}

Eq.~\ref{eq:21} further concludes that \brand will fall back to the Dense SGD 
approach in case 
of only one worker ($i.e. \;P=1$)

\paragraph{Theorem 2.} Assume that $g_t \in \mathbb{R}^m$  follows a 
bell-shaped distribution and $\pi^2$ is convex and less than the line 
$y=-i/m+1$ 
then we have $\parallel g^P_t \parallel = -i/m + 1$, then we have - 
\begin{equation}
\parallel g^P_t- \mathit{\mathbf{a2compress}}(g^P_t) \parallel^2 \le 
\{\frac{g_t^P}{\parallel g^P_t \parallel^2} - 1 +
\frac{\Aop(g_t^P)}{\parallel g^P_t \parallel^2} - 
\frac{\frac{1}{P}\sum_{p=1}^{P}\Aop(g_t^p)}{\parallel g^P_t \parallel^2}\} 
\parallel g^P_t \parallel^2 \label{eq:22}
\end{equation}

Furthermore it can be reorganized as-
\begin{equation}
\parallel g^P_t- \mathit{\mathbf{a2compress}}(g^P_t) \parallel^2 \le 
(1-\nabla \mu_{t})\parallel g^P_t \parallel^2,\label{eq:23}
\end{equation}

\begin{equation}
(1-\nabla \mu_{t})=
\{\frac{g_t^P}{\parallel g^P_t \parallel^2} - 1 +
\frac{\Aop(g_t^P)}{\parallel g^P_t \parallel^2} - 
\frac{\frac{1}{P}\sum_{p=1}^{P}\Aop(g_t^p)}{\parallel g^P_t \parallel^2}\} 
\label{eq:23}
\end{equation}

\begin{equation}
\nabla \mu_{t}=
\{2 - \frac{g_t^P}{\parallel g^P_t \parallel^2} -
\frac{\Aop(g_t^P)}{\parallel g^P_t \parallel^2} + 
\frac{\frac{1}{P}\sum_{p=1}^{P}\Aop(g_t^p)}{\parallel g^P_t \parallel^2}\} 
\label{eq:23}
\end{equation}

Hence, from Theorem. 2~\ref{eq:23} and  using Remark 4. from 
~\citet{karimireddy2019error}, we can derive the following Theorem-

\paragraph{Theorem 3.}
If we set $\eta_t = \frac{1}{\sqrt{T+1}}$ for running \brand and under the 
following assumption-
\begin{itemize}
	\item $C$ is \textit{L-smooth}
	\item $C$ has a moment bound ($i.e, \Expect{g} = \Delta_wC(w)\; \textit{and 
	}	\Expect{\parallel g \parallel^2} \le G^2\; \textit{for some 
	}\;G>0\textit{, 
		where g is the stochastic gradient and w is the model parameter}$)
\end{itemize}

We can state the following-
\begin{equation}
\min_{t \epsilon [T]} \Expect{\parallel \Delta_wC(w) \parallel^2} \le 
\frac{4(C(w) - w*) + LG^2}{2\sqrt{T+1}} + 
\frac{4L^2G^2(1-\nabla \mu_{t})}{\nabla \mu_{t}^2(T+1)} \label{eq:24}
\end{equation}

\begin{displaymath}
\mathrm{\mathbf{where}}\; \nabla \mu_{t} = \{2 - 
\frac{g_t^P}{\parallel g^P_t \parallel^2} -
\frac{\Aop(g_t^P)}{\parallel g^P_t \parallel^2} + 
\frac{\frac{1}{P}\sum_{p=1}^{P}\Aop(g_t^p)}{\parallel g^P_t \parallel^2}\} 
\end{displaymath}
\begin{center}
	\&,
\end{center}
\begin{displaymath}
\frac{1}{\nabla \mu_{t}^2} = 
\frac{1}{\{2 
	- \frac{g_t^P}{\parallel g^P_t \parallel^2} -
	\frac{\Aop(g_t^P)}{\parallel g^P_t \parallel^2} + 
	\frac{\frac{1}{P}\sum_{p=1}^{P}\Aop(g_t^p)}{\parallel g^P_t 
	\parallel^2}\}^2}
\end{displaymath}


Hence, the variance bound of our approach, $\nabla \mu_{t}$ is defined as:
$\{2 
- \frac{g_t^P}{\parallel g^P_t \parallel^2} -
\frac{\Aop(g_t^P)}{\parallel g^P_t \parallel^2} + 
\frac{\frac{1}{P}\sum_{p=1}^{P}\Aop(g_t^P)}{\parallel g^P_t 
	\parallel^2}\}^2$
and after $T \ge \Or(\frac{1}{\{2 
	- \frac{g_t^P}{\parallel g^P_t \parallel^2} -
	\frac{\Aop(g_t^P)}{\parallel g^P_t \parallel^2} + 
	\frac{\frac{1}{P}\sum_{p=1}^{P}\Aop(g_t^P)}{\parallel g^P_t 
		\parallel^2}\}^2})$ iterations, the first term of the right hand 
side of the Eq.~\ref{eq:24} will dominate the bound which will result in 
the convergence rate of $\Or(\frac{1}{\sqrt{T}})$ [same as vanilla 
SGD] afterwards.

--Texts written here are for my own understanding. ignore it..
In the convention minibatch gradient descent with one process will determine 
the number of iterations for each epoch by dividing the total training samples 
by the batchsize. After each iterations, the model weights are updated using 
the generated gradient based on back-propagation.

Now, when we distribute the entire method in data parallel approach, each 
iteration gets divided among the workers. So, if the number of worker is $N$, 
each worker will process batch-size/$N$ amount of samples per iteration. So, 
basically we split an iteration of processing multiple batches into workers. 
After the forward pass of pernode batch of sample a set of gradient gets 
generated in worker. To maintain the consistency, the allreduce approach simply 
sum/average the gradient vectors of all nodes. So, the weight update is all 
nodes are consistent in this case i.e, if weight 0 of worker 0 is decreased by 
x, the weight 0 of other workers also get decreased by x. 

However, we propose a different weight update strategy. Instead of updating 
consistent graidents across all nodes, we first take average of the gradients 
in each worker and keep the difference from the average as residuals. Finally, 
we add residuals with the allreduced value and update the weight with the 
result. 

We know from bengio and glorot and several other papers that the gradients show 
bell shaped distribution over iteration. As our approach follows the same 
distribution property, it should converge according to Gaussian K paper.

Now, what is the convergence rate. We closely look at the TernGrad paper, 
they derive the convergence rate from ...

First, we will derive an operator-
\end{comment}
\paragraph{Remark 2.}
The value of 

\begin{equation}
\nabla \mu_{t} = (\bar{\mu}_{t} - \Aop(g_t)) 
\end{equation}
\begin{displaymath}
= \lbrack \{pos(g_t) 
\cdot 
\bar{\mu}_{t,+}\; - \;neg(g_t) \cdot \bar{\mu}_{t,-}\}\;\; - \;\;\{
pos(g_t) 
\cdot \mu_{t,+}\; - \;neg(g_t) \cdot \mu_{-}\}\rbrack
\end{displaymath}
\begin{displaymath}
= \lbrack \{pos(g_t) \cdot 
(\bar{\mu}_{t,+} - {\mu}_{t,+}) - neg(g_t) \cdot 
(\bar{\mu}_{t,-} - {\mu}_{t,-})\}\rbrack
\end{displaymath}
\begin{equation}
\frac{1}{\nabla \mu_{t}} =  \frac{1}{\lbrack \{pos(g_t) \cdot 
	(\bar{\mu}_{t,+} - {\mu}_{t,+}) - neg(g_t) \cdot 
	(\bar{\mu}_{t,-} - {\mu}_{t,-})\}\rbrack}\end{equation}
\begin{equation}\frac{1}{(\nabla \mu_{t})^2} =  \frac{1}{\lbrack 
\{pos(g_t) \cdot 
	(\bar{\mu}_{t,+} - {\mu}_{t,+}) - neg(g_t) \cdot 
	(\bar{\mu}_{t,-} - {\mu}_{t,-})\}\rbrack^2} \end{equation}

Also, if we consider our operator as \textbf{<\;For validation check only with 
	the 
	operator suggested by Dr. Yu\;>}
\begin{equation}
\Aop (g^P_t) =
\begin{cases}
& \mu(g^P_t) \;\;\;\;\;\;\;\;\forall{g^P_t} \ge 0\\
& \mu(g^P_t) \;\;\;\;\;\;\;\; 	otherwise
\end{cases}    \label{eq:1}   
\end{equation}
The value of

\begin{equation}
\nabla \mu_{t} = \lbrack\{\Aop 
(g^P_t) - \frac{1}{P}\sum_{p=1}^{P} \Aop (g^P_t)\}\rbrack
\end{equation}
\begin{equation}
\frac{1}{\nabla \mu_{t}} =  \frac{1}{\lbrack \{\Aop 
	(g^P_t) - \frac{1}{P}\sum_{p=1}^{P} \Aop 
	(g^P_t)\}\rbrack}\end{equation}
\begin{equation}\frac{1}{(\nabla \mu_{t})^2} = 
\frac{1}{\lbrack\{\Aop 
	(g^P_t) - \frac{1}{P}\sum_{p=1}^{P} \Aop (g^P_t)\}\rbrack^2} 
\end{equation}
*Just a comment: Maybe evitable feature relation with worker.
If we can divide \textbf{"the number of batches and the features \textit{as 
per 
}batchsize per node"} it will mimic that feature

\textbf{
Reference to prove theorem 2: 
\[
https://en.wikipedia.org/wiki/68-95-99.7\_rule\#Cumulative\_distribution\_function\]
Very close to the concept of the notion of confidence interval
}

Usually if we do not tune anything, some errors $(\bar{\mu_t} -  
 \Aop (g^P_t))$ will 
be 
accumulated in distributed batch setting. The error is distributed 
batch 
setting thus can also be analyzed for its bound. For single worker, there will 
be no error bound as our approach will fall back to dense SGD.
\paragraph{Lemma 1.} If $g_t \in \mathbb{R}^m$  follows a bell-shaped 
distribution and $\Aop$ denotes the gradient distribution in \brand approach, 
then we have - 

\begin{equation}
\parallel g_t - \Aop(g_t) \parallel^2 \le (1-\nabla \mu_{t})\parallel g_t 
\parallel^2 
\label{eq:22}
\end{equation}
Proof-

Statement to be proven:$
\parallel g_t - \Aop(g_t) \parallel^2 \le (1-\nabla \mu_{t})\parallel g_t 
\parallel^2%,\;\;\;\;\;\;\; 
%\mathit{\mathbf{where}}\; \nabla \mu_{t} = \frac{\nabla \mu_{t} 
%}{g_t}
\label{eq:23}
$

First consider the mean and variance of the bell-shaped curve used in Vanilla 
distributed SGD with gradient vector $g_t^P$-

Mean of the gradient distribution: $\mu_1 = \frac{1}{P}\sum_{p=1}^{P}g_t^p$ = 
Gradient produced in Dense SGD

Variance of the gradient distribution: $\sigma_1 = \parallel g_t^P \parallel^2$


%Now calculate the mean and variance of our distribution:

%Using Eq:~\ref{eq:4}, we will calculate the mean and variance of our 
%distribution of gradient vector-

Now, we will calculate the exact distance between the spread of Dense SGD and 
\brand

$\mu_2 = g_t^P - \Aop(g_t^P) + \frac{1}{P}\sum_{P=1}^P \Aop (g^p_t)$

Variance of \brand gradient distribution: $\sigma_2 = \parallel g_t^P 
\parallel^2$ 
as variance of $\Aop$ operator is zero as it returns mean always.

distance between the two spread(Dense SGD in distributed node and $\Aop$) then 
can be calculated as-

$distance= (\mu_1 + 2\sigma_1) - (\mu_2 + 2\sigma_2)  = (\mu_1 - \mu_2)$,
where sigma is the standard deviation of the that distribution and 
$\sigma_1=\sigma_2=\parallel g_t \parallel^2$ if we look closely into the 
dense distributed SGD and dense \brand approach.

Hence, from Theorem. 2~\ref{eq:23} and  using Remark 4. and Remark 5. from 
~\citet{karimireddy2019error}, we can derive the following Theorem-

\paragraph{Theorem 3.}
If we set $\eta_t = \frac{1}{\sqrt{T+1}}$ for running \brand and under the 
following assumption-
\begin{itemize}
	\item $C$ is \textit{L-smooth}
	\item $C$ has a moment bound ($i.e, \Expect{g} = \Delta_wC(w)\; \textit{and 
	}	\Expect{\parallel g \parallel^2} \le G^2\; \textit{for some 
	}\;G>0\textit{, 
	where g is the stochastic gradient and w is the model parameter}$)
\end{itemize}

We can state the following-
\begin{equation}
\min_{t \epsilon [T]} \Expect{\parallel \Delta_wC(w) \parallel^2} \le 
\frac{4(C(w) - w*) + LG^2}{2\sqrt{T+1}} + 
\frac{4L^2G^2(1-\nabla \mu_{t})}{\nabla \mu_{t}^2(T+1)} \label{eq:24}
\end{equation}
\begin{comment}
\begin{displaymath}
\mathrm{\mathbf{where}}\; \nabla \mu_{t} = \frac{\nabla \mu_{t} }{g_t}
\end{displaymath}
\begin{center}
	\&,
\end{center}
\begin{displaymath}
\frac{1-\nabla \mu_{t}}{\nabla \mu_{t}^2} = \frac{g_t + \nabla \mu_{t} 
}{(\frac{\nabla \mu_{t} 
}{g_t})^2}
\end{displaymath}
\end{comment}

Hence, the variance bound of our approach, $\nabla \mu_{t}$ is defined as:
$\lbrack \{pos(g_t) \cdot (\bar{\mu}_{t,+} - {\mu}_{t,+}) - neg(g_t) 
\cdot(\bar{\mu}_{t,-} - {\mu}_{t,-})\}\rbrack$ or $\lbrack \{\Aop 
	(g^P_t) - \frac{1}{P}\sum_{p=1}^{P} \Aop 
	(g^P_t)\}\rbrack$ and after $T \ge \Or(\frac{1}{\lbrack 
	\{pos(g_t) \cdot 
	(\bar{\mu}_{t,+} - {\mu}_{t,+}) - neg(g_t) \cdot 
	(\bar{\mu}_{t,-} - {\mu}_{t,-})\}\rbrack^2})$ or $T \ge 
	\Or(\frac{1}{\lbrack\{\Aop (g^P_t) - 
\frac{1}{P}\sum_{p=1}^{P} \Aop 
(g^P_t)\}\rbrack^2})$iterations, the first term of 
the right hand 
	side of the Eq.~\ref{eq:24} will dominate the bound which will result in 
	the convergence rate of $\Or(\frac{1}{\sqrt{T}})$ [same as vanilla 
	SGD] afterwards.
Our bound is more strickter than other schemes as it ensures same convergence 
rate for a single worer while ensuring little higher error bound than dense SGD 
if we do not tune the per Worker Batch Size/Learning Rate explicitly for 
distributed training.


==> text/convergence_subhadeep.tex <==
\paragraph{Discussion.}
Normal distribution with mean $\mu$ and standard deviation $\sigma$ can 
be 
represented as $\mu + z\sigma$. According to Empirical/Three-Sigma rule in 
statistics, 
for the 
value of $z$ as 2 and 3 almost 95\% and 99.7\% gradient points
will fall under the curve and the subsequent calculations respectively. We will 
discuss about two distributions here. 
\textbf{Distribution 1} 
represents 
Distributed Dense SGD approach while \textbf{Distribution 2} is for \brand 
approach-

\textbf{Distribution 1: Distributed Dense SGD}

\textit{Assume normal distribution of values in a gradient $g_t$ of $d$ 
	dimensions
	$(g^1_t, g^2_t, ..., g^d_t)$ in distributed Dense SGD approach with mean 
	$\mu_1$ and variance $\sigma_1^2$.}
\begin{equation}
\parallel g_t \parallel = \mu_1 + z\sigma_1
\end{equation}
\textbf{Distribution 2: \brand}

\textit{Assume normal distribution of values in a gradient $g_t^\prime$ of $d$ 
	dimensions $(g^{\prime 1}_t, g^{\prime 2}_t, ..., g^{\prime d}_t)$ in 
	\brand approach with mean 
	$\mu_2$ and variance $\sigma_2^2$}
\begin{equation}
\parallel g_t^\prime \parallel = \mu_2 + z\sigma_2
\end{equation}

In A2SGD approach, the variance remains same: 
$\sigma_1^2 = \sigma_2^2$ 
which implies, $\sigma_1 = \sigma_2$, where $\sigma_1$ represents the standard 
deviation of Gradient values before allreduce(which is also equals to the 
gradients generated in Distributed Dense SGD approach) and $\sigma_2$ 
represents the standard deviation of final gradient values in \brand approach 
after 
allreduce.

Distance between the distributions $= \parallel g_t - g_t^\prime \parallel = 
(\mu_1 + z\sigma_1) - 
(\mu_2 + z\sigma_2)  = (\mu_1 - \mu_2)$,
as $\sigma_1=\sigma_2$.

%sigma is the 
%standard deviation of the that 
%distribution and 
%=\parallel g_t \parallel^2$ if we look closely into the 
%dense distributed SGD and dense \brand approach.

%$\mu_2 = g_t^P - \Aop(g_t^P) + \frac{1}{P}\sum_{P=1}^P \Aop (g^p_t)$

%Variance of \brand gradient distribution: $\sigma_2 $
%\begin{comment}
%= \parallel g_t^P 
%\parallel^2$ 
%as variance of $\Aop$ operator is zero [it returns mean always]
%\end{comment}
Hence, we can write the following:
\begin{equation}
\parallel g_t - g_t^\prime\parallel^2 = (\mu_1 - \mu_2)^2
\end{equation}

\paragraph{Convergence Rate.}
Based on the previous studies, we evaluate the relation between $\parallel g_t 
- g_t^\prime \parallel^2$ and 
$\parallel g_t \parallel^2$:

\textbf{Objective:} \textit{Find the value of $\delta$ where,
	\begin{equation}
	\parallel g_t - g_t^\prime \parallel^2 = (1-\delta) \parallel g_t 
	\parallel^2
	\end{equation}}

\textbf{Solution:}

\begin{displaymath}
(1-\delta)\parallel g_t \parallel^2 = (\mu_1 - \mu_2)^2
\end{displaymath}
\begin{displaymath}
1-\delta = \frac{(\mu_1 - \mu_2)^2}{\parallel g_t \parallel^2}
\end{displaymath}
\begin{displaymath}
\delta = 1 - \frac{(\mu_1 - \mu_2)^2}{\parallel g_t \parallel^2} = 
\frac{\parallel g_t \parallel^2 - (\mu_1 - \mu_2)^2}{\parallel g_t \parallel^2}
\end{displaymath}

\textit{So, following Remarks 4. of ~\citeauthor{karimireddy2019error}, we can 
	directly 
	write 
	the following -}

\paragraph{Theorem 2.}
If we set $\eta_t = \frac{1}{\sqrt{T+1}}$ for running \brand and under the 
following assumption-
\begin{itemize}
	\item $C$ is \textit{L-smooth}
	\item $C$ has a moment bound ($i.e, \Expect{g} = \Delta_wC(w)\; \textit{and 
	}	\Expect{\parallel g \parallel^2} \le G^2\; \textit{for some 
	}\;G>0\textit{, 
		where g is the stochastic gradient and w is the model parameter}$)
\end{itemize}

\textit{We can state the following-}
\begin{equation}
\min_{t \epsilon [T]} \Expect{\parallel \Delta_wC(w) \parallel^2} \le 
\frac{4(C(w) - w^*) + LG^2}{2\sqrt{T+1}} + 
\frac{4L^2G^2(1-\delta)}{\delta(T+1)} \label{eq:24}
\end{equation}

\textit{where} $\delta = \frac{\parallel g_t \parallel^2 - (\mu_1 - 
	\mu_2)^2}{\parallel g_t \parallel^2}$%\\
%$= \frac{-2\parallel g_t \parallel(\parallel g_t \parallel - 
%\parallel g_t^\prime \parallel) - n(\mu^{\prime 
%	2} - 2\mu\mu^\prime)}{\parallel g_t 
%\parallel^2}$

Hence, the variance bound of our approach, $\delta$ is defined as:
$ \delta = \frac{\parallel g_t \parallel^2 - (\mu_1 - \mu_2)^2}{\parallel g_t 
	\parallel^2} $ and 
after $T \ge \Or(\frac{\parallel g_t \parallel^2}{\parallel g_t \parallel^2 - 
	(\mu_1 - \mu_2)^2})$iterations, the first term of 
the right hand 
side of the Eq.~\ref{eq:24} will dominate the bound which will result in 
the convergence rate of $\Or(\frac{1}{\sqrt{T}})$ [same as vanilla 
SGD] afterwards.
Our bound is more strict than other schemes as it ensures \textbf{same 
convergence 
rate for a single worker}.

\paragraph{More strict bound than others: (Definition of $\mu_1$ and $\mu_2$)}
We further want to exploit the definition of convergence rate by evaluating it 
in terms of original gradient value $g_t$ with dimension $d$:

$\mu_1$ can be written as: $\frac{1}{d}\sum_{i=1}^{d}g_t^i$

$\mu_2$ can be written as: $\frac{1}{d}\sum_{i=1}^{d}(g_t^i + \nabla\mu_t)$

Hence, the convergence bound can be further expressed as:

\begin{equation}
\Or(\frac{\parallel g_t \parallel^2}{\parallel g_t 
\parallel^2 - (\frac{1}{d}\sum_{i=1}^{d}g_t - \frac{1}{d}\sum_{i=1}^{d}(g_t + 
\nabla\mu_t))^2})\label{eq:rate}
\end{equation}

Hence, it is more evident from Equation~\ref{eq:rate} that when the value of 
$\nabla\mu_t$(The net gain) will become $0$, the convergence rate will be 
similar as Dense SGD approach. 

\begin{equation}
\nabla \mu_{t} = (\bar{\mu}_{t} - \Aop(g_t)) 
\end{equation}
\begin{displaymath}
= \lbrack \{pos(g_t) 
\cdot 
\bar{\mu}_{t,+}\; - \;neg(g_t) \cdot \bar{\mu}_{t,-}\}\;\; - \;\;\{
pos(g_t) 
\cdot \mu_{t,+}\; - \;neg(g_t) \cdot \mu_{-}\}\rbrack
\end{displaymath}
\begin{displaymath}
= \lbrack \{pos(g_t) \cdot 
(\bar{\mu}_{t,+} - {\mu}_{t,+})\} - \{neg(g_t) \cdot 
(\bar{\mu}_{t,-} - {\mu}_{t,-})\}\rbrack
\end{displaymath}

Moreover, it also shows that, if the absolute mean before 
allreduce(${\mu}_{t,sign}$) and the absolute mean after 
allreduce($\bar{\mu}_{t,sign}$) 
becomes equal, the 
convergence rate will follow that of a single worker Batch Gradient Descent.
 

==> text/design-backup.tex <==
\section{Design of Distributed SGD with Two-Level Gradient Averaging}
%\section{Two-Level Gradient-Averaged SGD}

\paragraph{Distribution of Gradients.}
Most of the previous sparsification and quantization related studies focus on selecting the most significant portion of gradients either in terms of magnitude or in terms of elements respectively, as they contribute more to the updates. Hence, it is necessary to analyze the gradient distribution of Dense SGD carefully. Initially, extensive experiments have been conducted to analyze the overall gradient distribution in different deep learning models and three representative datasets have been chosen from the category of FNNs(Feed-forward Neural Networks), CNNs(Convolution Neural Networks), and RNNs(Recurrent Neural Networks) to check the generality of gradient distributions. As shown from ~\ref{fig:gradient_distribution}, the gradient distribution always follows the bell-shaped curve of the normal distribution, and most of the gradients clustered around zero. So, instead of directly discarding some elements like sparsification approaches, a new approach has been introduced to maintain the entire \textbf{distribution of data}.
Moreover, in quantization approaches, the determination of the exact 
quantization level involves several hyper-parameter tuning, and also, the 
accuracy drops with the increase in quantization level. Sparsification 
approaches follow a similar trend as the accuracy of the model drops with a 
decrease in the size of selected gradients. So, in both of the approaches, a 
part of the variance of the gradient data after sparsification/quantization is 
lost, which contributes to the overall accuracy difference with Dense SGD and 
convergence rate. Furthermore, the proposed approach tries to minimize the loss 
in variance to provide an excellent convergence rate and better accuracy with 
minimal gradient exchange.

\begin{figure}[H]
	\centering
	\begin{subfigure}[b]{0.25\textwidth}
		\centering
		\includegraphics[width=\textwidth]{./evaluation/fnn3_density.pdf}
		\caption{FNN3 Density}
		\label{fig:fnn3_density}
	\end{subfigure}%
	~
	\begin{subfigure}[b]{0.224\textwidth}
		\centering
		\includegraphics[width=\textwidth]{./evaluation/fnn3_hist.pdf}
		\caption{FNN3 Histogram}
		\label{fig:vgg16_density}
	\end{subfigure}%
	~
	\begin{subfigure}[b]{0.25\textwidth}
		\centering
		\includegraphics[width=\textwidth]{./evaluation/resnet20_density.pdf}
		\caption{ResNet20 Density}
		\label{fig:resnet20_density}
	\end{subfigure}%
	~
	\begin{subfigure}[b]{0.224\textwidth}
		\centering
		\includegraphics[width=\textwidth]{./evaluation/resnet20_hist.pdf}
		\caption{ResNet20 Histogram}
		\label{fig:resnet20_hist}
	\end{subfigure}\\
	\caption{This plot demonstrates Gradient Density of last iteration for 
	A1SGD, \brand and Dense SGD. Also, the progression of Gradient Frequency 
	Distribution in 
	\textit{\brand}approach	across iterations are shown alongside. }
	\label{fig:hist_density}
\end{figure}

\paragraph{Distributed SGD with Gradient Averaging.}
The overall design of our method tries to communicate the minimal number of 
data for all reduction while ensuring a better convergence rate and similar 
convergence loss as Dense SGD. To contain the maximum variation within data, we 
tried to send only the mean of the entire gradient distribution for all to 
reduce while keeping the difference between each sample of gradient 
distribution and the mean as residuals. After the entire reduction is 
completed, the residual for each sample is added back to the all reduce mean to 
generate the updated tensor values. Although this approach gives us 
considerable performance improvement in terms of accuracy and scalability of 
the FNN and CNN training, it does not work well with RNNs. After careful 
examination of gradient distribution of the last iteration as showed in 
~\ref{fig:hist_density}, we can see that range of Dense SGD data in the rug 
plot of RNNs is much more concentrated in around zero whereas for A1SGD it is 
spread. Averaging of entire gradient distribution works well with FNNs and CNNs 
as the range of the gradient data is smaller than RNNs. To overcome this issue, 
we implement Distributed SGD with two levels, which is described in the 
following subsection.

\begin{comment}
\begin{figure}[!htb]
	\begin{center}
		\subfigure[{\ttfamily FNN3-MNIST}\label{fig:fnn3_density}]
		{\includegraphics[width=0.32\textwidth]{./evaluation/convergence/vgg16-8worker_accuracy.pdf}}
		\subfigure[{\ttfamily VGG16-CIFAR10}\label{fig:vgg16_density}]
		{\includegraphics[width=0.32\textwidth]{./evaluation/convergence/vgg16-8worker_accuracy.pdf}}
		\subfigure[{\ttfamily LSTM-PTB}\label{fig:lstm_density}]
		{\includegraphics[width=0.32\textwidth]{./evaluation/convergence/vgg16-8worker_accuracy.pdf}}
		\caption{Gradient Density<Placeholder>}
		\label{fig:gradient_density}
	\end{center}
\end{figure}
\end{comment}
\paragraph{Distributed SGD with Two-Level Gradient Averaging.}
\brand first divides the entire gradient distribution into two subsets based on 
their $sign(.)$ values to segregate positive and negative values in two pools. 
Then we calculate the pooled average of the pools as mentioned earlier and 
store the residuals similar to A1SGD. Instead of exchanging only a single mean 
from each worker for all reduce, each worker sends the mean from each pull for 
all reduce. The negative means are all reduced with negative mean values of a 
worker, and the positive means are all reduced with positive means of the 
worker. Again after the all reduce completes, the residuals of negative pools 
are added back to the all reduced negative mean and vice-versa to generate the 
updated gradients. As shown in ~\ref{fig:hist_density}, the rug plot shows the 
data are showing almost similar density to Dense SGD. As most of the values are 
either on both sides of zeros, AISGD unable to capture maximum variance and 
vanishes some of the gradients because of the positive and negative signs. 
Furthermore, in the case of RNN, it is still unable to achieve a similar 
density as dense version as the gradient distribution is much more spread than 
CNNs. So, it is evident that increasing the number of pools can help RNN to 
achieve similar distribution as the dense version.

\begin{comment}

Placeholder for design(3.25 pages including 2 pages convergence analysis)

Design Plan:

\begin{itemize}
\item Motivation for top-1 val accuracy (2 worker with batchsize 1024) -- val acc  vs EPOCH - Dense K, TopK, Gaussian TopK
\subitem FNN3 on MNIST -- Need to fix today
\subitem RESNET20 on CIFAR10 -- Need to fix today
\subitem LSTM on PTB -- Need to fix today
\subitem AlexNet on ImageNet -- maybe later

\item Justification about overall weight distribution (Follows TernGrad paper section 3.3 - we will not show layerwise) - Ours only
\subitem VGG16 on CIFAR10 - Communication intensive (More CNV layers)
\subitem AlexNet on ImageNet - Computation intensive (More fully connected layers) -- maybe later

\item GPU Computation time - (vary gradient range from 1x1e8 to 16x1e8) -- Next
\subitem TopK
\subitem Gaussian K
\subitem Ours

\item Plot 3(b) from Gaussian K - Use Ref line, Gaussian TopK and Ours
4.1 VGG16 on CIFAR10 --- Not needed

\item CDF plot Gardients- iteration [200, 400, 800, 1200, 1600] -- We will not plot CDF instead we will do rug plot

\subitem VGG16 on CIFAR10
\subitem RESNET20 on CIFAR10
\subitem AlexNet on ImageNet
\end{itemize}
\end{comment}
\input{text/algorithm.tex}


\input{text/convproof.tex}

%\input{text/convergence.tex}
%\input{text/rateproof.tex}


==> text/impact.tex <==
\section*{Broader Impact}

Our proposed A2SGD algorithm will have broader impact to the field of 
high-performance deep learning through distributed SGD, particularly on the
use of big neural network models and the deployment of large-scale computer
systems and high-speed networks.  With its dramatic reduction on the
communication complexity of gradient synchronization, A2SGD will propel the
adoption of big DNN models for a wide variety of image classification, speed
recognition and natural language processing applications.  In addition, with its
demonstrated scalability, it will promote the use of large-scale
computer systems for deep learning. Furthermore, its reduction on
communication traffic per worker can dampen the system administrators and practitioners 
seeking to deploy large-scale high-bandwidth communication networks for deep learning.
On the other hand, A2SGD can encourage the deployment of deep learning models on
low-bandwidth computing systems such as IoT (Internet of Things) and Edge Computing environments. 

We also acknowledge that A2SGD is an initial prototype that can be refined
further, e.g., the addition of an Allgather implementation as noted in the paper.
In addition, we are yet to systematically document the importance of
hyperparameters in A2SGD in comparison to other algorithms. Thus our reported
results can have some bias towards A2SGD which is the focal point of our training.
Thus we also plan to analyze and document the impact of various hyperparameters. 


==> text/newproof.tex <==
\subsection{Rate Analysis}

\begin{comment}
\begin{equation}
\parallel g_t + \nabla \mu_{t} \parallel^2\; = \;\parallel g_t \parallel^2 
\;\;\;\;
\iff\;\; \Aop(g_t) = \bar \mu_{t} \label{eq:21}
\end{equation}

Eq.~\ref{eq:20} further concludes that \brand will fall back to the Dense SGD approach in case 
of only one worker ($i.e. \;P=1$) since $\nabla \mu_{t} = 0 $.
\end{comment}

\paragraph{Discussion: Local Error is zero.}

Based on prior studies and our own profile, we can assume 
the gradient values in a gradient vector $g_t$  = 
$(g^1_t, g^2_t, ..., g^n_t)$ at the $t$-th iteration 
follow a standard normal distribution $(\mu_t, \sigma_t^2)$.

\textit{We can compute the following Variance,} 

\begin{equation}
\sigma_t^2 = \frac{\sum_{i=1}^{n}g_t^i}{n} 
= \mathbb{E}(g_t^{2}) - [\mathbb{E}(g_t)]^2 
= \frac{\parallel g_t \parallel^2}{n} - \mu_t^2 
\end{equation}

Thus we can represent the second moment of $g_t$ as follows.

\begin{equation}
\parallel g_t \parallel^2 = n \cdot (\mu_t^2 + \sigma_t^2) 
= n \cdot \sigma_t^2, \label{equ:moment}
\end{equation}

assuming $\mu_t \to 0$ for the standard normal distribution.

In the \brand algorithm, we compute and exchange the local means for positive
and negative values. We can assume that both positive and negative values in 
$g_t$ follow half normal distribution, where we can denote 
the positive half as ($\mu_{t,+}, \sigma_{t,+}^2$) and 
the negative half as ($\mu_{t,-}, \sigma_{t,-}^2$).

Hence, we can have these equality equations. 

\begin{equation}
|\mu_t - \mu_{t,-} |  = |\mu_t - \mu_{t,+}|  = \frac{\sigma\sqrt{2}}{\sqrt{\pi}},
\end{equation}
   and 
\begin{equation}
\sigma_{t,-}^{2} = \sigma_{t,+}^{2} = \sigma_t^2 \cdot (1 - \frac{2}{\pi}).
\end{equation}

As described earlier, in each iteration, gradient $g_t$ substracts its own
means and then gains back the global means. 
We can denote $\nabla \mu_{t,+} = \bar{\mu}_{t,+}-\mu_{t,+}$
and $\nabla \mu_{t,-} = \bar{\mu}_{t,-}-\mu_{t,-}$ 
as the net gain on the positive and negative means, 
respectively.
In addition, we can denote $\bar{\mu}_{t} = pos(g_t) \cdot \bar{\mu}_{t,+} 
- neg(g_t) \cdot \bar{\mu}_{t,-}$ as the vector composed global means.
Essentially, $\nabla \mu_{t} = \bar{\mu}_{t} - \Aop(g_t)$ is the net gain.

Since the global positive mean $\bar{\mu}_{t,+}$ is the mean of the local
means from $P$ workers, it can be perceived as a sample with P equal subsets.
Thus the variance of local positive means is reduced by $P$ times with $P$ equal subsets.

\begin{equation}
\bar{\sigma}_{t,+}^{2} = \frac{\sigma_{t,+}^{2}}{P} = \frac{\pi-2}{P\pi} \sigma_t^2.
\label{equ:subpos}
\end{equation}

Similarly, we have the variance of local negative means is reduced by $P$ times with $P$ equal subsets.

\begin{equation}
\bar{\sigma}_{t,-}^{2} = \frac{\sigma_{t,-}^{2}}{P} = \frac{\pi-2}{P\pi} \sigma_t^2.
\label{equ:subneg}
\end{equation}


Let us denote the updated gradient as $g_t^\prime = g_t + \nabla \mu_{t}$.
Essentially, for each half of the gradient $g_t$, we shift their values twice.
Shifting the mean does not change the variance of any distribution. 

The expection of L2 norm for the new gradient
values after allreduce in \brand approach can be defined as.

%\begin{equation}
%	\parallel g_t^\prime \parallel^2 = \{\sigma_t^2 + (\mu_t - \mu^\prime)^2\}n =
%	\{\sigma^2 + (\mu^2 + \mu^{\prime 2} - 2\mu\mu^{\prime})\}n = 
%	\parallel 
%	g_t \parallel^2+ n(\mu^{\prime 2} - 2\mu\mu^\prime)\label{eq:a8}
%\end{equation}

\begin{equation}
	\parallel g_t^\prime \parallel^2 = \parallel g_t + \nabla \mu_{t} \parallel^2 \label{eq:a8}
\end{equation}

Compared to quantization and sparsification techniques that compress the
gradient for synchronization, \brand only shifts the means. While each half of the
gradient did not change its variance, the total variance and the moment 
of $g_t$ still change. Thus it is
important to understand its important on the moment. 

\begin{equation}
\parallel g_t - g_t^\prime \parallel^2 =  \parallel \nabla \mu_{t} \parallel^2
\end{equation}

Since $\nabla \mu_{t}$ represents the shifted means for each half normal
distribution, we can evaluate the change on the moment from $g_t$ to $g_t^\prime$
as follows.

\textbf{Solution:}

\begin{equation}
\parallel \nabla \mu_{t} \parallel^2 = 
\sum_{i=1}^{\frac{n}{2}} |\bar{\mu}_{t,-} - \mu_{t,-}|^2 
+ \sum_{i=1}^{\frac{n}{2}} |\bar{\mu}_{t,+} - \mu_{t,+}|^2
= 
\frac{n}{2P}\sum_{i=1}^{P} |\bar{\mu}_{t,-} - \mu_{t,-}|^2 
+ \frac{n}{2P}\sum_{i=1}^{P} |\bar{\mu}_{t,+} - \mu_{t,+}|^2 
%= \frac{n}{2P}\sigma_{t,-}^{2} + \frac{n}{2P}\sigma_{t,+}^{2} 
%= \frac{n}{P} \sigma_t^2 \cdot (1 - \frac{2}{\pi}).
%\sigma_t^2 = \frac{\sum_{i=1}^{n}g_t^i}{n} 
%= \frac{n (\pi - 2 ) }{P\pi}\sigma_t^2.
\end{equation}

\begin{equation}
\parallel \nabla \mu_{t} \parallel^2 
= \frac{n}{2P}(P\bar{\sigma}_{t,-}^{2} + P\bar{\sigma}_{t,+}^{2})
= \frac{n}{2P}(\sigma_{t,-}^{2} + \sigma_{t,+}^{2})
= \frac{n}{P} \sigma_t^2 \cdot (1 - \frac{2}{\pi})
%\sigma_t^2 = \frac{\sum_{i=1}^{n}g_t^i}{n} 
= \frac{\pi - 2}{\pi P}(n \cdot \sigma_t^2)
= \frac{\pi - 2}{\pi P} \parallel g_t \parallel^2,
\end{equation}

where the second equality was based on Equ.~\ref{equ:subpos} and Equ.~\ref{equ:subneg},
the last equality based on Equ.~\ref{equ:moment}.

We can introduce a parameter $\delta$ to represent the moment change,

\begin{equation}
\parallel g_t - g_t^\prime \parallel^2 =  (1-\delta) \parallel g_t \parallel^2  
= \frac{\pi - 2}{\pi P} \parallel g_t \parallel^2 .
\end{equation}

Solving the equation, we can derive the value of $\delta$ as follows.

\begin{equation}
\delta = 1 - \frac{\pi - 2}{\pi P}.
\end{equation}

Following the example of~\citet{karimireddy2019error}, we can make two more assumptions. 

\paragraph{Assumption B} (Smoothness). A function $f: \mathbb{R}^n \to \mathbb{R}$ 
is $L$-smooth if for all x, y $\in \mathbb{R}^n $, the following
holds.

\begin{equation}
| f(y) - (f(x) + \nabla f(x)^T \cdot (y - x) ) | \leq \frac{L}{2} \parallel y - x \parallel^2
\end{equation}

\paragraph{Assumption C} (Moment bound). For any query (training) of a
stochastic gradient, SGD returns a gradient $g$ such that 
\begin{equation}
\mathbb{E}[g] = \nabla f(x), and \;\;
\mathbb{E}\parallel g \parallel^2 \leq \phi^2.
\end{equation}

\paragraph{Theorem 2} (Non-convex convergence of \brand). 
Let $\{w_t\}_{t\geq 0}$ denote an iteration of \brand for 
any step-size $\eta > 0$. Under Assumptions A, B, and C,

    \begin{equation}
    \min\limits_{t \in [T]} \mathbb{E}[\parallel \nabla f(w_t) \parallel^2 ] 
    \leq \frac{2 f_0}{\eta (T+1)} + \frac{\eta L \phi^2}{2} + unknown,
    \end{equation}

with $f_0 := f(w_0) - f^*$.

\paragraph{Proof Sketch}. 
Intuitively, the condition that $\mathcal{C}(\cdot)$ is a $\delta$-approximate compressor implies that at each
iteration a $\delta$-fraction of the gradient information is sent. The rest is added to et to be transmitted later.
Eventually, all the gradient information is transmitted—albeit with a delay
which depends on $\delta$. Thus \brand can intuitively be viewed as a delayed gradient method. 
If the function is smooth, the gradient does not change quickly and so the delay does not significantly matter.

\paragraph{Proof:} 

\begin{equation}
f(w_{t+1}) 
\leq f(w_t) + \nabla f(w_t)^T \cdot (w_{t+1} - w_t) + \frac{L}{2} \parallel w_{t+1} - w_t \parallel^2
\end{equation}

For the dense SGD case with one worker, we would not exchange the local means and
introduce no gains on the computed gradient, hence $w_{t+1} = w_t - \eta \nabla f(w_t)$.

\begin{equation}
f(w_{t+1}) 
\leq f(w_t) - \eta \nabla f(w_t)^T \mathbb{E}_t ([g_t]) + \frac{L\eta^2}{2} \parallel
g_t \parallel^2. %(since \; w_{t+1} = w_t - \eta \nabla f(w_t))
\end{equation}

\begin{equation}
f(w_{t+1}) 
\leq f(w_t) - \eta \nabla f(w_t)^T \nabla f(w_t)  + \frac{L\eta^2}{2} \parallel g_t \parallel^2 
= f(w_t) - \eta \parallel \nabla f(w_t) \parallel^2 + \frac{L\eta^2}{2} \phi^2  
\end{equation}


Rearrange the terms and take average over t, we can have the following equations.

\begin{equation}
\eta \parallel \nabla f(w_t) \parallel^2 \leq f(w_{t}) - f(w_{t+1}) + \frac{L\eta^2}{2} \phi^2  
\end{equation}

\begin{equation}
\frac{1}{T+1}\sum_{i=0}^{T} \parallel \nabla f(w_t) \parallel^2 
\leq \frac{1}{\eta(T+1)}\sum_{i=0}^{T} (f(w_{t}) - f(w_{t+1})) + \frac{L\eta}{2} \phi^2  
\leq \frac{1}{\eta(T+1)} (f(x_{0}) - f^{*}) + \frac{L\eta}{2} \phi^2  
\end{equation}

This proves Theorem 2 for the dense SGD case.
\begin{equation}
\min\limits_{t \in [T]} \mathbb{E}[\parallel \nabla f(x_t) \parallel^2 ] 
\leq \frac{2 f_0}{\eta (T+1)} + \frac{\eta L \phi^2}{2},
\end{equation}

with $f_0 := f(w_0) - f^*$.

For \brand with P worker, we would exchange the local means and
introduce no gains on the computed gradient, hence 
$w_{t+1} = w_t - \eta (\nabla f(w_t) - \nabla \mu_t)$.
We can prove Theorem 2 as follows.



==> text/rateproof.tex <==
\subsection{Rate Analysis}

%If we apply the notion of a compressor from Stitch et al.~\cite{},
%the compressor from A2SGD will have this property.
%compared to the no

\paragraph{Discussion: Local Error is zero.}
We will discuss about two distributions here. Case 1 denotes the gradients 
$g_t$ generated by the Distributed Dense approach and Case 2 illustrates the 
properties of gradients generated by \brand approach.

\textbf{Case 1:}

\textit{Assume normal distribution of values in a gradient $g_t$ of $d$ 
dimensions
$(g^1_t, g^2_t, ..., g^n_t)$ in distributed Dense SGD approach, where $g^i_t$ 
follows standard Normal
distribution $(\mu, \sigma^2)$.}

\textit{We can compute the following Variance,} $ \sigma^2 = 
\frac{\sum_{i=1}^{n}g_t^i}{n} = 
\mathbb{E}(g_t^{2}) - 
[\mathbb{E}(g_t)]^2 = \frac{\parallel g_t \parallel^2}{n} - \mu^2 $

$ \parallel g_t \parallel^2 = n * (\mu^2 + \sigma^2) $.

\textbf{Case 2:}

\textit{In case of \brand, we can assume that both positive and negative values 
in 
$g_t^\prime$ 
follow half normal distribution ($\mu^\prime, \sigma^{\prime2}$).}

\textit{Hence, $\mu^\prime - \mu$ = $\frac{\sigma\sqrt{2}}{\sqrt{\pi}}$, where 
$\mu^\prime$ and $\mu$ are the mean values of dense SGD and
variance, $\sigma^{\prime2} = \sigma^2 \cdot (1 - \frac{2}{\pi})$.}

\textit{When we subtract the mean $\mu^\prime$ before allreduce, we essentially 
shift 
each half of the normal distribution. This does not change its variance. 
However, the mean is changed.} 

\textit{The expection of L2 norm for the new gradient
values after allreduce in \brand approach can be defined as-}

\begin{equation}
	\parallel g_t^\prime \parallel^2 = \{\sigma^2 + (\mu - \mu^\prime)^2\}n =
	\{\sigma^2 + (\mu^2 + \mu^{\prime 2} - 2\mu\mu^{\prime})\}n = 
	\parallel 
	g_t \parallel^2+ n(\mu^{\prime 2} - 2\mu\mu^\prime)\label{eq:a8}
\end{equation}

\paragraph{Convergence Rate.}
Based on the previous studies, we evaluate the relation between $\parallel g_t 
- g_t^\prime \parallel^2$ (distance between $g_t$ and $g_t^\prime$) and 
$\parallel g_t \parallel^2$:

\textbf{Objective:} \textit{Find the value of $\delta$ where,
\begin{equation}
	\parallel g_t - g_t^\prime \parallel^2 = (1-\delta) \parallel g_t 
	\parallel^2
\end{equation}}

\textbf{Solution:}
\begin{equation}
\parallel g_t^\prime - g_t \parallel^2 = \parallel g_t^\prime \parallel^2 + 
\parallel g_t \parallel^2 - 
2\parallel g_t^\prime g_t \parallel \label{eq:a10}
\end{equation}

\textit{Based on the Eq:~\ref{eq:a8}, we replace $\parallel g_t \parallel^2$ in 
Eq.~\ref{eq:a10}}

\begin{displaymath}
= n(\mu^{\prime 2} - 2\mu\mu^\prime) + 
2\parallel g_t \parallel^2 - 
2\parallel g_t^\prime g_t \parallel = (2 - 
2\frac{\parallel g_t^\prime \parallel}{\parallel g_t \parallel} + 
\frac{n(\mu^{\prime 2} - 2\mu\mu^\prime)}{\parallel g_t \parallel^2}) 
\parallel 
g_t \parallel^2
\end{displaymath}

\begin{equation}
= \{1 - (-2 + 
2\frac{\parallel g_t^\prime \parallel}{\parallel g_t \parallel} - 
\frac{n(\mu^{\prime 2} - 2\mu\mu^\prime)}{\parallel g_t \parallel^2})\} 
\parallel 
g_t \parallel^2 = (1-\delta) \parallel g_t \parallel^2
\end{equation}

\textit{So, following Remarks 4. of ~\citeauthor{karimireddy2019error}, we can 
directly 
write 
the following -}

\paragraph{Theorem 2.}
If we set $\eta_t = \frac{1}{\sqrt{T+1}}$ for running \brand and under the 
following assumption-
\begin{itemize}
	\item $C$ is \textit{L-smooth}
	\item $C$ has a moment bound ($i.e, \Expect{g} = \Delta_wC(w)\; \textit{and 
	}	\Expect{\parallel g \parallel^2} \le G^2\; \textit{for some 
	}\;G>0\textit{, 
		where g is the stochastic gradient and w is the model parameter}$)
\end{itemize}

\textit{We can state the following-}
\begin{equation}
\min_{t \epsilon [T]} \Expect{\parallel \Delta_wC(w) \parallel^2} \le 
\frac{4(C(w) - w^*) + LG^2}{2\sqrt{T+1}} + 
\frac{4L^2G^2(1-\delta)}{\delta(T+1)} \label{eq:24}
\end{equation}

\textit{where} $\delta = -2 + 
2\frac{\parallel g_t^\prime \parallel}{\parallel g_t \parallel} - 
\frac{n(\mu^{\prime 2} - 2\mu\mu^\prime)}{\parallel g_t \parallel^2} = \frac{-2 
\parallel g_t \parallel^2 + 2\parallel g_t g_t^\prime \parallel - n(\mu^{\prime 
2} - 2\mu\mu^\prime)}{\parallel g_t 
\parallel^2} $%\\
%$= \frac{-2\parallel g_t \parallel(\parallel g_t \parallel - 
%\parallel g_t^\prime \parallel) - n(\mu^{\prime 
%	2} - 2\mu\mu^\prime)}{\parallel g_t 
%\parallel^2}$

Hence, the variance bound of our approach, $\delta$ is defined as:
$ \delta = \frac{-2 
	\parallel g_t \parallel^2 + 2\parallel g_t g_t^\prime \parallel - 
	n(\mu^{\prime 
		2} - 2\mu\mu^\prime)}{\parallel g_t 
	\parallel^2} $ and 
after $T \ge \Or(\frac{\parallel g_t 
	\parallel^2}{-2 
	\parallel g_t \parallel^2 + 2\parallel g_t g_t^\prime \parallel - 
	n(\mu^{\prime 
		2} - 2\mu\mu^\prime)})$iterations, the first term of 
the right hand 
side of the Eq.~\ref{eq:24} will dominate the bound which will result in 
the convergence rate of $\Or(\frac{1}{\sqrt{T}})$ [same as vanilla 
SGD] afterwards.
Our bound is more strickter than other schemes as it ensures same convergence 
rate for a single worer while ensuring little higher error bound than dense SGD 
if we do not tune the per Worker Batch Size/Learning Rate explicitly for 
distributed training.

\begin{comment}
The absolute means across P workers all follow half normal distributions.
We can calculate their average through allreduce. 
The expected value for the global mean will remain the same, but the variance
will be reduced by P times according to the rules regarding pooled samples, 
($\bar{\mu}^\prime, \bar{\sigma}^{\prime2}$), where 
$\bar{\mu}^\prime = \mu^\prime $, and $\bar{\sigma}^{\prime2} =
\sigma^{\prime2} / P$.}


\paragraph{Assumption 2 (Smoothness)

\paragraph{Theorem 4. (Convex Convergence of A2SGD)}

If we set $\eta_t = \frac{1}{\sqrt{T+1}}$ for running \brand and under the 
following assumption-
\begin{itemize}
	\item $C$ is \textit{L-smooth}
	\item $C$ has a moment bound ($i.e, \Expect{g} = \Delta_wC(w)\; \textit{and 
	}	\Expect{\parallel g \parallel^2} \le G^2\; \textit{for some 
	}\;G>0\textit{, 
	where g is the stochastic gradient and w is the model parameter}$)
\end{itemize}

We can state the following-
\begin{equation}
\min_{t \epsilon [T]} \Expect{\parallel \Delta_wC(w) \parallel^2} \le 
\frac{4(C(w) - w*) + LG^2}{2\sqrt{T+1}} + 
\frac{4L^2G^2(1-\nabla \mu_{t})}{\nabla \mu_{t}^2(T+1)} \label{eq:24}
\end{equation}

Hence, the variance bound of our approach, $\nabla \mu_{t}$ is defined as:
$\lbrack \{pos(g_t) \cdot (\bar{\mu}_{t,+} - {\mu}_{t,+}) - neg(g_t) 
\cdot(\bar{\mu}_{t,-} - {\mu}_{t,-})\}\rbrack$ or $\lbrack \{\Aop 
	(g^P_t) - \frac{1}{P}\sum_{p=1}^{P} \Aop 
	(g^P_t)\}\rbrack$ and after $T \ge \Or(\frac{1}{\lbrack 
	\{pos(g_t) \cdot 
	(\bar{\mu}_{t,+} - {\mu}_{t,+}) - neg(g_t) \cdot 
	(\bar{\mu}_{t,-} - {\mu}_{t,-})\}\rbrack^2})$ or $T \ge 
	\Or(\frac{1}{\lbrack\{\Aop (g^P_t) - 
\frac{1}{P}\sum_{p=1}^{P} \Aop 
(g^P_t)\}\rbrack^2})$iterations, the first term of 
the right hand 
	side of the Eq.~\ref{eq:24} will dominate the bound which will result in 
	the convergence rate of $\Or(\frac{1}{\sqrt{T}})$ [same as vanilla 
	SGD] afterwards.
Our bound is more strickter than other schemes as it ensures same convergence 
rate for a single worer while ensuring little higher error bound than dense SGD 
if we do not tune the per Worker Batch Size/Learning Rate explicitly for 
distributed training.
\end{comment}

